Secure Information Embedding in Forensic 3D Fingerprinting

Printer fingerprinting techniques have long played a critical role in forensic applications, including the tracking of counterfeiters and the safeguarding of confidential information. The rise of 3D printing technology introduces significant risks to public safety, enabling individuals with internet access and consumer-grade 3D printers to produce untraceable firearms, counterfeit products, and more. This growing threat calls for a better mechanism to track the production of 3D-printed parts. Inspired by the success of fingerprinting on traditional 2D printers, we introduce SIDE (\textbf{S}ecure \textbf{I}nformation Embe\textbf{D}ding and \textbf{E}xtraction), a novel fingerprinting framework tailored for 3D printing. SIDE addresses the adversarial challenges of 3D print forensics by offering both secure information embedding and extraction. First, through novel coding-theoretic techniques, SIDE is both~\emph{break-resilient} and~\emph{loss-tolerant}, enabling fingerprint recovery even if the adversary breaks the print into fragments and conceals a portion of them. Second, SIDE further leverages Trusted Execution Environments (TEE) to secure the fingerprint embedding process.

==> figures/rate-k-t.tex <==
\begin{tikzpicture}
\begin{axis}[
    title={Code rate~$t$ vs.~$k,t$},
    xlabel={Information length~$k$ },
    ylabel={code rate~$r=k/n$},
    xmin=0, xmax=400,
    ymin=.1, ymax=.6,  
    xtick={50,100,150,200,250,300,350,400},
    % ytick={0,200,400,600,800,1000},
    ytick={0,0.1,0.2,0.3,0.4,0.5,0.6},
    legend pos=north west,
    ymajorgrids=false,
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (191, 0.481)(203, 0.487)(215, 0.492)(227, 0.497)(239, 0.501)(251, 0.505)(263, 0.509)(275, 0.512)(287, 0.515)(299, 0.518)(311, 0.521)(323, 0.524)(335, 0.526)(347, 0.528)(359, 0.53)
    };  
\addlegendentry{$t=1$}

\addplot[
    color=red,
    mark=triangle,
    ]
    coordinates {
    (179, 0.394)(191, 0.403)(203, 0.411)(215, 0.418)(227, 0.425)(239, 0.431)(251, 0.437)(263, 0.443)(275, 0.448)(287, 0.453)(299, 0.457)(311, 0.461)(323, 0.465)(335, 0.469)(347, 0.473)
    };
\addlegendentry{$t=2$} 

\addplot[
    color=green,
    mark=o,
    ]
    coordinates {
    (167, 0.327)(179, 0.337)(191, 0.347)(203, 0.356)(215, 0.364)(227, 0.372)(239, 0.379)(251, 0.386)(263, 0.392)(275, 0.398)(287, 0.404)(299, 0.409)(311, 0.414)(323, 0.419)(335, 0.424)
    };
\addlegendentry{$t=3$}

\addplot[
    color=yellow,
    mark=+,
    ]
    coordinates {
    (155, 0.273)(167, 0.284)(179, 0.294)(191, 0.304)(203, 0.313)(215, 0.322)(227, 0.33)(239, 0.338)(251, 0.345)(263, 0.352)(275, 0.358)(287, 0.364)(299, 0.37)(311, 0.376)(323, 0.381)
    };
\addlegendentry{$t=4$}

\addplot[
    color=black,
    mark=star,
    ]
    coordinates {
    (143, 0.229)(155, 0.24)(167, 0.251)(179, 0.261)(191, 0.271)(203, 0.28)(215, 0.289)(227, 0.297)(239, 0.304)(251, 0.312)(263, 0.319)(275, 0.325)(287, 0.332)(299, 0.338)(311, 0.344)
    };
\addlegendentry{$t=5$}

\addplot[
    color=violet,
    mark=x,
    ]
    coordinates {
    (131, 0.192)(143, 0.204)(155, 0.215)(167, 0.225)(179, 0.235)(191, 0.244)(203, 0.253)(215, 0.262)(227, 0.27)(239, 0.277)(251, 0.285)(263, 0.292)(275, 0.298)(287, 0.305)(299, 0.311)
    };
\addlegendentry{$t=6$}


\addplot[
    color=cyan,
    mark=+,
    ]
    coordinates {
    (119, 0.161)(131, 0.173)(143, 0.184)(155, 0.194)(167, 0.204)(179, 0.213)(191, 0.222)(203, 0.231)(215, 0.239)(227, 0.247)(239, 0.255)(251, 0.262)(263, 0.269)(275, 0.275)(287, 0.282)
    };
\addlegendentry{$t=7$}

\addplot[
    color=magenta,
    mark=diamond,
    ]
    coordinates {
    (107, 0.134)(119, 0.146)(131, 0.157)(143, 0.167)(155, 0.177)(167, 0.186)(179, 0.195)(191, 0.204)(203, 0.212)(215, 0.22)(227, 0.228)(239, 0.235)(251, 0.242)(263, 0.249)(275, 0.256)
    };
\addlegendentry{$t=8$}

\addplot [
    domain=0:400, 
    samples=10, 
    color=red,
    ]
    {1/3};

\addplot [
    domain=0:400, 
    samples=10, 
    color=blue,
    ]
    {0.5};

\addplot [
    domain=0:400, 
    samples=10, 
    color=green,
    ]
    {0.25};

\addplot [
    domain=0:400, 
    samples=10, 
    color=yellow,
    ]
    {0.2};

\addplot [
    domain=0:400, 
    samples=10, 
    color=black,
    ]
    {1/6};

\addplot [
    domain=0:400, 
    samples=10, 
    color=violet,
    ]
    {1/7};

\addplot [
    domain=0:400, 
    samples=10, 
    color=cyan,
    ]
    {1/8};

\addplot [
    domain=0:400, 
    samples=10, 
    color=magenta,
    ]
    {1/9};

\end{axis}
\end{tikzpicture}

==> figures/tkn.tex <==
\begin{tikzpicture}
\begin{axis}[
    title={Demonstration of~$t,k,n$},
    xlabel={number of breaks~$t$ },
    ylabel={codeword length~$n$},
    xmin=0, xmax=9,
    % ymin=0, ymax=1000,
    ymin=0, ymax=1,    
    xtick={0,1,2,3,4,5,6,7,8,9},
    % ytick={0,200,400,600,800,1000},
    ytick={0,.200,.400,.600,.800,1},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
    ]
    % coordinates {
    % (1,211)(2,260)(3,327)(4,394)(5,461)(6,528)(7,595)(8,662)
    % };
    coordinates {
    (1,64/211)(2,64/260)(3,64/327)(4,64/394)(5,64/461)(6,64/528)(7,64/595)(8,64/662)
    };
    \addlegendentry{$k=64$}

\addplot[
    color=green,
    mark=triangle,
    ]
    % coordinates {
    % (1,247)(2,314)(3,381)(4,448)(5,515)(6,582)(7,739)(8,796)
    % };
    coordinates {
    (1,96/247)(2,96/314)(3,96/381)(4,96/448)(5,96/515)(6,96/582)(7,96/739)(8,96/796)
    };
    \addlegendentry{$k=96$}

\addplot[
    color=red,
    mark=star,
    ]
    % coordinates {
    % (1,301)(2,368)(3,435)(4,568)(5,625)(6,682)(7,759)(8,836)
    % };
    coordinates {
    (1,128/301)(2,128/368)(3,128/435)(4,128/568)(5,128/625)(6,128/682)(7,128/759)(8,128/836)
    };
    \addlegendentry{$k=128$}

\addplot[
    color=black,
    mark=x,
    ]
    % coordinates {
    % (1,397)(2,454)(3,511)(4,588)(5,665)(6,742)(7,819)(8,896)
    % };
    coordinates {
    (1,160/397)(2,160/454)(3,160/511)(4,160/588)(5,160/665)(6,160/742)(7,160/819)(8,160/896)
    };
    \addlegendentry{$k=160$}

\end{axis}
\end{tikzpicture}

==> revision_summary.tex <==

APPENDIX - Revision Summary 
“Secure Information Embedding in Forensic 3D Fingerprinting”

We appreciate the reviewers' constructive feedback on our previous manuscript draft and deeply value the opportunity to enhance our work. Below, we summarize the changes made:

RC1: Better motivate the validity of disabling vulnerable components

We added a subsection in Section 3, “Motivation and Related,” to motivate the validity of disabling vulnerable components. Specifically, 

We introduced the necessity of fault tolerance in CPS design. 

We included a survey study of fault tolerance in the four CPS platforms tested in this paper to demonstrate its general applicability.

We introduced the simplex architecture, which is the fault-tolerance paradigm that inspired Gecko’s design.

Additionally, in the design of shadow compartments (Section 4.2), we also discuss how the built-in fault tolerance can be used as shadow compartments.


Changes can be found in Section 2.3 and Section 4.2. 


RC2  -  xxx


Other Changes

We refined the design figures to improve clarity. 


RC1: Textual revision: Clarify the threat model and assumptions. Expand discussion on forging attack. Provide justification for high code rate necessity.

We will revise to include the followings: Threat model and assumptions: We will clarify assumptions about an attacker's capabilities, including the use of hardware equipped with SIDE and the threshold for the number of hidden or broken pieces in 3D printing objects. We will also note that stopping omnipotent adversaries is impossible. However, regulating manufacturers to include SIDE in commercial 3D printers and requiring attackers to break objects into multiple pieces or hide more pieces to bypass fingerprinting would significantly raise the bar for criminal activities. Discussion on forging attacks: We will discuss forging attacks and potential solutions, such as authenticating the print by embedding the hash of intrinsic printer properties in the security analysis. Justification for high code rate necessity: We will justify the necessity of a high code rate in the revision by discussing potential forensic applications that could benefit from a higher code rate.

RC2: New Experiments

RC2.1: Conduct print quality evaluation using existing 3D printing benchmarks, such as 3D Benchy. SIDE embeds information by varying layer thickness, which influences surface roughness. To quantify this impact, we plan to employ optical coherence tomography (OCT) to capture the deviations in surface height of printed objects. The collected data is used to compute the root mean square (RMS) roughness value, a widely adopted metric for surface roughness that represents the root mean square of surface height deviations from the mean surface height [1][2]. To evaluate the quality of 3D-printed objects produced with SIDE, we compare the RMS roughness of SIDE-printed objects (3DBenchy) to that of objects printed without SIDE. [1] Gadelmawla, Elamir S., et al. "Roughness parameters." Journal of materials processing Technology 123.1 (2002): 133-145. [2] Wi, Kwangwoo, et al. "Quantifying quality of 3D printed clay objects using a 3D structured light scanning system." Additive Manufacturing 32 (2020): 100987.

RC2.2: Analyze impacts of important factors, including printer imperfection, number of breaks (>8), fragment loss, and the size and shape of printed objects. We use a combination of real-world experiments and simulations to analyze the impact of printer imperfection, number of breaks (>8), fragment loss, and the size and shape of printed objects.

Impact of printer imperfection: We will conduct real-world experiments to evaluate how printer imperfections affect information embedding. Specifically, we will measure the success rate of correct information extraction from objects produced by imperfect 3D printers. In each experiment, we will simulate printer imperfections by adjusting calibration parameters (e.g., the number of stepper motor steps required to lift the nozzle by 1 mm).
Impact of Fragment Loss, Number of Breaks, and Size/Shape of Printed Objects: We will conduct simulation-based experiments to analyze the effects of fragment loss, number of breaks, and the size and shape of printed objects. Each experiment will focus on one of 3D models with distinct shapes (including 3DBenchy, AR-15 lower receiver, and the FMDA Glock Frame used in the killing of Brian Thompson, CEO of UnitedHealthcare), subjected to a series of fracture simulations. Specifically, the 3D model will be randomly divided into pieces, and we will test whether the fingerprint can be recovered from only a subset of these fragments. The experiments will systematically vary the object size, number of breaks, number of omitted pieces, and the security threshold of BRC, observing their impact on the success rate of fingerprint recovery.
RC2.3: Validate the feasibility of the stealthy fingerprinting method proposed in the response.

To validate the proposed stealthy fingerprinting mechanism, we will evaluate its stealthiness by comparing it with the bit embedding method proposed in the manuscript that comes without the stealthiness mechanism. We measure stealthiness by evaluating the surface roughness of the prints. A surface roughness closer to that of prints without bit embedding indicates higher stealthiness. Meanwhile, we will verify the success of bit extraction under the stealthy fingerprinting mechanism.

RC2.4: Perform system performance evaluation for the TEE implementation.

To assess the performance impact of TEE implementations in SIDE, we measure the runtime and memory overhead of a 3D printing application under both micro and macro benchmark perspectives, with and without TEE. Furthermore, we evaluate the effects of TEE implementations on the printing process.

Micro benchmark: We will measure the execution delays of four functional modules running in TEE, including codec, layer generation, toolpath generation, and firmware execution within the TEE when printing 3D objects.

Macro benchmark: We will measure the execution delay and memory overhead involved in printing 3D objects, both with and without the TEE implementation from SIDE, to demonstrate the effectiveness of runtime heap memory reduction achieved by our automatic model split tools.

Impact on printed objects: We will measure the surface roughness of 3D objects printed by applications running with and without the TEE implementation in SIDE.

RC2.5: Determine and validate minimum object size requirements for successful SIDE fingerprinting.

The theoretical minimum object size is determined by the bit embedding granularity (i.e., millimeters per bit) and the length of the BRC codeword. The codeword length, in turn, is a function of the number of fingerprint bits and the security parameter (t) of the BRC. Essentially, BRC requires extra redundant bits to provide enhanced robustness against breaks, i.e., the number of breaks that can be tolerated, since one extra break leads to at most two additional errors in the data structure~
next
next. This inevitably results in longer codewords. We will revise to include the formula that calculates the minimum object size in paper.

To validate the theoretical boundary, we will print the 3D objects with minimized size and corresponding BRC codewords embedded and observe from optical coherence tomography to verify whether the expected information can be accurately extracted from the printed objects.

Individual Comments: In addition to the listed revision criteria, we will also try our best to address individual comments.

Submission Time: We decide to submit it on Jan 9th.
